MlTr: Multi-label Classification with Transformer

The task of multi-label image classification is to recognize all the object labels presented in an image. Though advancing for years, small objects, similar objects and objects with high conditional probability are still the main bottlenecks of previous convolutional neural network(CNN) based models, limited by convolutional kernels' representational capacity. Recent vision transformer networks utilize the self-attention mechanism to extract the feature of pixel granularity, which expresses richer local semantic information, while is insufficient for mining global spatial dependence. In this paper, we point out the three crucial problems that CNN-based methods encounter and explore the possibility of conducting specific transformer modules to settle them. We put forward a Multi-label Transformer architecture(MlTr) constructed with windows partitioning, in-window pixel attention, cross-window attention, particularly improving the performance of multi-label image classification tasks. The proposed MlTr shows state-of-the-art results on various prevalent multi-label datasets such as MS-COCO, Pascal-VOC, and NUS-WIDE with 88.5%, 95.8%, and 65.5% respectively. The code will be available soon at https://github.com/starmemda/MlTr/

==> remain.tex <==
\textbf{Arc sigmoid.}
The most widely used multi-label classification loss function, bce loss, is presented as follows:
\begin{eqnarray}
L_i = -\sum_{j}^{n}{y_{ij}}\log\frac{1}{1+e^{x_{i}W_j^T+b_j}}-\sum_{j}^{n}{(1-y_{ij})}\log\frac{1}{1+e^{-x_{i}W_j^T-b_j}}
\end{eqnarray}
where $x \in \mathbb{R}^{N\times{d}}$ denotes the features extracted by model in $N$ samples and d means the feature dimension which often set to 2048 in these paper following. $i$ means i-th sample and $j$ means j-th class.So $W_j \in \mathbb{R}^{d}$ and $b_j \in \mathbb{R}^{d}$ denotes the j-th column of the weight of $W \in \mathbb{R}^{d\times{n}}$
and bias item in the final fully connected layer. True label we want the model to learn is y.\\
We can infer that $W_j$ is the most typical feature of the j-th category, which is represented in the form of vector in the d-dimensional hyperplane space. When the product of feature $x_i$ and $W_j$ learned by the model from an image reaches the maximum, we will make the i-th sample's predicted score in the j-th category as the maximum. Referring to the paper\cite{deng2019arcface,liu2017sphereface,liu2016large}, we believe that it is more reasonable to describe the similarity among vectors by the angle on the hyperplane, so we put forward the arc sigmoid function which expresses as belows:
\begin{eqnarray}
\label{arc sigmoid}
L_i = -\sum_{j}^{n}{y_{ij}}\log\frac{1}{1+e^{s\cos\theta}}-\sum_{j}^{n}{(1-y_{ij})}\log\frac{1}{1+e^{-s\cos\theta}}
\end{eqnarray}
where $\theta = \arccos\frac{x_{i}W_j^T}{||x_{i}||||W_j^T||}$ exactly means the angle among vector $x_{i}$ and $W_i^T$, s is a superparameter used to keep the predicted value within $[-s, s]$.\\\\
